Explainable Metric Learning for Deflating Data Bias

Image classification is an essential part of computer vision which assigns a given input image to a specific category based on the similarity evaluation within given criteria. While promising classifiers can be obtained through deep learning models, these approaches lack explainability, where the classification results are hard to interpret in a human-understandable way. In this paper, we present an explainable metric learning framework, which constructs hierarchical levels of semantic segments of an image for better interpretability. The key methodology involves a bottom-up learning strategy, starting by training the local metric learning model for the individual segments and then combining segments to compose comprehensive metrics in a tree. Specifically, our approach enables a more human-understandable similarity measurement between two images based on the semantic segments within it, which can be utilized to generate new samples to reduce bias in a training dataset. Extensive experimental evaluation demonstrates that the proposed approach can drastically improve model accuracy compared with state-of-the-art methods.

==> sec/0_abstract.tex <==
\begin{abstract}
Image classification is an essential part of computer vision which assigns a given input image to a specific category based on the similarity evaluation within given criteria. While promising classifiers can be obtained through deep learning models, these approaches lack explainability, where the classification results are hard to interpret in a human-understandable way. In this paper, we present an explainable metric learning framework, which constructs hierarchical levels of semantic segments of an image for better interpretability. The key methodology involves a bottom-up learning strategy, starting by training the local metric learning model for the individual segments and then combining segments to compose comprehensive metrics in a tree. Specifically, our approach enables a more human-understandable similarity measurement between two images based on the semantic segments within it, which can be utilized to generate new samples to reduce bias in a training dataset. Extensive experimental evaluation demonstrates that the proposed approach can drastically improve model accuracy compared with state-of-the-art methods.
% Additionally, this approach introduces minor overhead as a tradeoff for better model accuracy and interpretable similarity measurements.
\end{abstract}

==> sec/preliminary.tex <==
\section{Generalized Preliminaries}
Let $D$ be the image dataset as a collection of instances, each can be represented as a feature vector $x_i$ in the feature space $X$. Formally, $D = \{(x_1,y_1), (x_2,y_2), ..., (x_N,y_N)\}$, where $N$ is the number of images, and $y_i$ is the corresponding label for $x_i$.

\noindent {\bf Metric Learning: }In the context of metric learning, a metric $d$ is defined as function $d: X \times X \rightarrow \mathbb{R}^+$ to measure the similarity or dissimilarity between two instances, which should satisfy the non-negativity, symmetry, and triangle inequality. Then a metric learning algorithm can be justified as a parameterized optimization process that minimizes a loss function over pairs or triplets of instances.
\[
min_\theta \sum_{x_i \sim x_j } d^2(x_i,x_j) + \lambda \sum_{x_i \not\sim x_j } d^2(x_i,x_j)
\]
which, in laymen terms, encourages the embedding of similar instances to be close together in the feature space.

\noindent {\bf Semantics :  }The semantic refers to a specific embedding section of images in the feature space or any projected space, and a similarity function $S(x_i, x_j)$ is defined to quantify the semantic similarity between them. It can be a function based on domain-specific knowledge or learned from data. For example, in natural language processing, the cosine similarity between word embeddings is often used as a measure of semantic similarity.
\[
S(x_i,x_j) = \frac{E(x_i)\cdot E(x_j)}{||E(x_i)|| \cdot ||E(x_j)||}
\]


\noindent {\bf Semantically Guided Metric Learning: } refers to a metric learning approach that incorporates semantic information into the learning process, which involves combining traditional distance metrics with semantic similarity measures. Commonly, the loss function for semantically guided metric learning can be generalized as 
\[
\mathcal{L}_{sem}(x_i,x_j, S(x_i,x_j))= d(x_i,x_j) - \alpha \cdot log(S(x_i,x_j))   
\]
where $\alpha$ is a weighting parameter.

\noindent {\bf A Tree-like hierarchical machine learning model} $T$ can be mathematically represented as a tuple: $T = (N,H,E)$ where $N$ is the set of nodes which is semantic model in our method as described in Section~\ref{sec:ss},$H$ defines the hierarchy which is demonstrated in Section~\ref{sec:bup}, and $E$ is the set of edges which is the way of tree composition presented in Section~\ref{sec:tree}. 

\noindent {\bf Explainability} refers to interpret the decisions or predictions made by a model. In this paper, we focus on \textit{global explainability} where we measuring the importance of each feature in the model's decision-making process. Basically, for a model $f$ and input $a = (a_1,a_2,...a-j)$ it can be viewed as 
$
Importance(a) = \sum_j \frac{\partial f(x)}{\partial x_{ij}}
$

We will show how we expand these fundamental concepts and how they were applied in our proposed explainable metric learning framework in next section.
